Ethereum's Recursive Length Prefix in ACL2

Recursive Length Prefix (RLP) is used to encode a wide variety of data in Ethereum, including transactions. The work described in this paper provides a formal specification of RLP encoding and a verified implementation of RLP decoding, developed in the ACL2 theorem prover. This work has led to improvements to the Ethereum documentation and additions to the Ethereum test suite.

==> eptcsdata.tex <==
\providecommand{\firstpage}{108}
\providecommand{\publicationstatus}{G. Passmore, R. Gamboa (Eds.): ACL2 Workshop 2020\\
EPTCS 327, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.327.11}{10.4204/EPTCS.327.11}}
\pdfoutput=1

